Model-based RL as a Minimalist Approach to Horizon-Free and Second-Order Bounds

Learning a transition model via Maximum Likelihood Estimation (MLE) followed by planning inside the learned model is perhaps the most standard and simplest Model-based Reinforcement Learning (RL) framework. In this work, we show that such a simple Model-based RL scheme, when equipped with optimistic and pessimistic planning procedures, achieves strong regret and sample complexity bounds in online and offline RL settings. Particularly, we demonstrate that under the conditions where the trajectory-wise reward is normalized between zero and one and the transition is time-homogenous, it achieves nearly horizon-free and second-order bounds. Nearly horizon-free means that our bounds have no polynomial dependence on the horizon of the Markov Decision Process. A second-order bound is a type of instance-dependent bound that scales with respect to the variances of the returns of the policies which can be small when the system is nearly deterministic and (or) the optimal policy has small values. We highlight that our algorithms are simple, fairly standard, and indeed have been extensively studied in the RL literature: they learn a model via MLE, build a version space around the MLE solution, and perform optimistic or pessimistic planning depending on whether operating in the online or offline mode. These algorithms do not rely on additional specialized algorithmic designs such as learning variances and performing variance-weighted learning and thus can easily leverage non-linear function approximations. The simplicity of the algorithms also implies that our horizon-free and second-order regret analysis is actually standard and mainly follows the general framework of optimism/pessimism in the face of uncertainty.

==> app_offline_new.tex <==
\section{Detailed Proofs for the Offline RL setting}


% \wen{give the MLE bound below in an independent lemma.}

% \zhiyong{Should we put it here? I think it is also used in online part} \wen{i see, let's maybe put a very general version in the supporting lemma section, and later just call it in each section when needed? }




\subsection{Proof of \pref{thm:mleoffline}}\label{app:offline}
The following is the full proof of \pref{thm:mleoffline}. 

% \wen{let's use the pref thing that i was using for consistency? i.e., \pref{thm:}}
[Proof of \pref{thm:mleoffline}]
    First, by the realizability assumption, and the standard generalization bound for MLE (\pref{lem:mle_generalization_offline}), we have that w.p. at least $1-\delta$: \\
    \begin{enumerate}
    \item[(1)] $P^\star\in\widehat\Pcal$; 
    \item[(2)]         \begin{equation}
            \sum_{h=0}^{H-1}\EE_{s,a\sim d^{\pi^b}_h}[\mathbb H^2(P^\star(s,a)||\widehat P(s,a))]\leq\frac{22\log(\left|\Pcal\right|/\delta)}{K}.\label{eqn: generalization offline}
        \end{equation}
        \end{enumerate}
        % (1) $P^\star\in\widehat\Pcal$; \\
        % (2) 
        % \begin{equation}
        %     \sum_{h=0}^{H-1}\EE_{s,a\sim d^{\pi^b}_h}[H^2(P^\star(s,a)||\widehat P(s,a))]\leq\frac{22\log(\left|\Pcal\right|/\delta)}{N}.\label{eqn: generalization offline}
        % \end{equation}
        
        % \wen{I changed $\hat P$ to $\widehat P $, @zhiyong, can you make them consistent in the proof?}
        
Then, with the above realizability in (1), and by the pessimistic algorithm design $\hat\pi\leftarrow \argmax_{\pi\in\Pi}\min_{P\in\widehat\Pcal} V_{0; P}^\pi(s_0)$, $\widehat P\leftarrow \argmin_{P \in \widehat \Pcal} V_{0; P}^{\widehat \pi}(s_0)$, we have that for any $\pi^\star\in\Pi$
\begin{align}
    V_{0; P^\star}^{\pi^\star}-V_{0; P^\star}^{\hat{\pi}}&=V_{0; P^\star}^{\pi^\star}-V_{0;\widehat P}^{\pi^\star}+V_{0;\widehat P}^{\pi^\star}-V_{0; P^\star}^{\hat{\pi}}\notag\\
    &\leq V_{0; P^\star}^{\pi^\star}-V_{0;\widehat P}^{\pi^\star}+V_{0;\widehat P}^{\hat{\pi}}-V_{0; P^\star}^{\hat{\pi}}\notag\\
    &\leq V_{0; P^\star}^{\pi^\star}-V_{0;\widehat P}^{\pi^\star}\,. \label{offline gap 1}
\end{align}
We can then bound $V_{0; P^\star}^{\pi^\star}-V_{0;\widehat P}^{\pi^\star}$ using the simulation lemma (\pref{lem:simulation}):
\dongruo{change here}
\begin{align}
    V_{0; P^\star}^{\pi^\star}-V_{0;\widehat P}^{\pi^\star}&\leq \sum_{h=0}^{H-1} \EE_{s,a\sim d^{\pi^\star}_h} \left[ \left|\EE_{s'\sim P^\star(s,a)} V^{\pi^\star}_{h+1;\widehat P}(s') -\EE_{s'\sim \widehat P(s,a)} V^{\pi^\star}_{h+1;\widehat P}(s')    \right|\right]\notag \\
\end{align}
We denote the offline data to be
\begin{align}
    \Dcal = \{(s_1^1, a_1^1, r_1^1,\dots, s_H^K, a_H^K, r_H^K)\},\ n = HK.
\end{align}


From here, we bound $\sum_{h=0}^{H-1}\EE_{s,a\sim d^{\pi^*}_h}$ with 
\begin{align}
    \frac{1}{K}\sum_{h=0}^{H-1}\sum_{k=1}^K \EE_{s\sim P^*(s_{h-1}^k, a_{h-1}^k), a \sim \pi^*(s)}\left[ \left|\EE_{s'\sim P^\star(s,a)} V^{\pi^\star}_{h+1;\widehat P}(s') -\EE_{s'\sim \widehat P(s,a)} V^{\pi^\star}_{h+1;\widehat P}(s')    \right|\right]\label{help:1}
\end{align}
We use Lemma \ref{lemma:new1}. 
First we forget about the error term and just replace it with \eqref{help:1}. Then we have
\begin{align}
    \eqref{help:1} &\leq  8\frac{1}{K}\sum_{h=0}^{H-1}\sum_{k=1}^K \EE_{s\sim P^*(s_{h-1}^k, a_{h-1}^k), a \sim \pi^*(s)} \left[\sqrt{\big(\VV_{P^\star} V_{h+1; \widehat P}^{\pi^\star}\big)(s,a)\mathbb H^2\Big(P^\star(s,a)\Mid \widehat P\big(s,a)\Big)}\right]\notag \\
    &+4\frac{1}{K}\sum_{h=0}^{H-1}\sum_{k=1}^K \EE_{s\sim P^*(s_{h-1}^k, a_{h-1}^k), a \sim \pi^*(s)}\left[\mathbb H^2\Big(P^\star(s,a)\Mid \widehat P\big(s,a)\Big)\right]\notag\\
    &\leq  \left[\sqrt{8\frac{1}{K}\sum_{h=0}^{H-1}\sum_{k=1}^K \EE_{s\sim P^*(s_{h-1}^k, a_{h-1}^k), a \sim \pi^*(s)} \big(\VV_{P^\star} V_{h+1; \widehat P}^{\pi^\star}\big)(s,a) \cdot 8\frac{1}{K}\sum_{h=0}^{H-1}\sum_{k=1}^K \EE_{s\sim P^*(s_{h-1}^k, a_{h-1}^k), a \sim \pi^*(s)} \mathbb H^2\Big(P^\star(s,a)\Mid \widehat P\big(s,a)\Big)}\right]\notag \\
    &+4\frac{1}{K}\sum_{h=0}^{H-1}\sum_{k=1}^K \EE_{s\sim P^*(s_{h-1}^k, a_{h-1}^k), a \sim \pi^*(s)}\left[\mathbb H^2\Big(P^\star(s,a)\Mid \widehat P\big(s,a)\Big)\right]\label{help:2}
\end{align}

By our MLE generalization lemma, we have
\begin{align}
    &\frac{1}{K}\sum_{h=0}^{H-1}\sum_{k=1}^K \EE_{s\sim P^*(s_{h-1}^k, a_{h-1}^k), a \sim \pi^b(s)}\left[\mathbb H^2\Big(P^\star(s,a)\Mid \widehat P\big(s,a)\Big)\right] \notag\\
    &=H\cdot \EE_{s,a\sim \frac{1}{HK} \left(\sum_{k=1}^K\sum_{h=0}^{H-1}P^*(s_{h-1}^k, a_{h-1}^k\right), a \sim \pi^b(s))}\left[\mathbb H^2\Big(P^\star(s,a)\Mid \widehat P\big(s,a)\Big)\right] 
    \leq \frac{\log(|\Pcal|/\delta)}{K}. 
\end{align}
We want to bound
\begin{align}
\sum_{h=0}^{H-1} \EE_{s,a \sim d^{\pi^\star}_h}\left[\mathbb H^2\Big(P^\star(s,a)\Mid \widehat P\big(s,a)\Big)\right]=H\cdot\EE_{s,a \sim 1/H\cdot \sum_{h=0}^{H-1} d^{\pi^\star}_h}\left[\mathbb H^2\Big(P^\star(s,a)\Mid \widehat P\big(s,a)\Big)\right]
\end{align}
Does it make sense to define the coverage as follows
% \begin{align}
%     \EE_{s,a \sim 1/H\cdot \sum_{h=0}^{H-1} d^{\pi^\star}_h} f(s,a)\leq C\cdot \EE_{s,a \sim 1/HK\cdot \sum_{k=1}^K\sum_{h=0}^{H-1} \Dcal_{h,k}} f(s,a)
% \end{align}

\begin{align*}
C^{\pi^*} := \max_{P \in \Pcal}  \frac{  \EE_{s,a \sim 1/H\cdot \sum_{h=0}^{H-1} d^{\pi^\star}_h} \mathbb{H}^2\left( P(s,a) \Mid P^\star(s,a) \right)   }{ \EE_{s,a\sim \frac{1}{HK} \left(\sum_{k=1}^K\sum_{h=0}^{H-1}P^*(s_{h-1}^k, a_{h-1}^k\right), a \sim \pi^b(s))} \mathbb H^2\left(   P(s,a)  \Mid   P^\star(s,a)  \right)    } . 
\end{align*}
\begin{align*}
C^{\pi^*} := \max_{P \in \Pcal}  \frac{  \EE_{s,a \sim 1/H\cdot \sum_{h=0}^{H-1} d^{\pi^\star}_h} \mathbb{H}^2\left( P(s,a) \Mid P^\star(s,a) \right)   }{ \min_{s }\EE_{a \sim \pi^b(s )} \mathbb H^2\left(   P(s ,a )  \Mid   P^\star(s ,a )  \right)    } . 
\end{align*}
For online, we have
\begin{equation}
    \sum_{i=0}^{k-1} \sum_{h=1}^H E_{s_h\sim P^*(s_{h-1}^i,a_{h-1}^i),a_h\sim\pi^i} H^2(P^k(s_h,a_h)||P^*(s_h,a_h))\leq \log(K|P|/\delta)
\end{equation}

and we need
% \begin{equation}
%     \sum_{i=0}^{k-1} \sum_{h=1}^H E_{(s_h,a_h)\sim d^{\pi^i}_h} H^2(P^k(s_h,a_h)||P^*(s_h,a_h))\leq \log(K|P|/\delta)
% \end{equation}

% To further prove
\begin{equation}
    \sum_{k=0}^{k-1} \sum_{h=1}^H E_{(s_h,a_h)\sim d^{\pi^k}_h} H^2(P^k(s_h,a_h)||P^*(s_h,a_h))\leq \log(K|P|/\delta)\times d_{RL}
\end{equation}
Should we define $f^k(\tau)=1/H \sum_{s,a \in \tau} H^2(P^k(s,a)||P^*(s,a))$? In this way, by MLE we can have $\sum_{i<k} f^k(\tau^i)\leq \log(K|P|/\delta)/H$ and then bound $\sum_{t=1}^k f^t(\tau^t)$ by $\log(K|P|/\delta)/H+1$, but we need $H\sum_{t=1}^k f^t(\tau^t)$, which is $\log(K|P|/\delta)+H$


\begin{lemma}\label{lemma:new1}
    Over the randomness of $\Dcal$, for some function $f_{\Dcal}(s,a)$ with probability at least $1-\delta$, 
\begin{align}
    \frac{1}{K}\sum_{h=0}^{H-1}\sum_{k=1}^K \EE_{s\sim P^*(s_{h-1}^k, a_{h-1}^k), a \sim \pi^b(s)}f_{\Dcal}(s,a) - \sum_{h=0}^{H-1}\EE_{s,a\sim d^{\pi^b}_h} f_{\Dcal}(s,a) \leq \sum_{h=0}^{H-1} \frac{\text{vsr}_{s,a\sim d^{\pi^b}_h} f_{\Dcal}(s,a)}{\sqrt{K}}\log(\Ncal/\delta) + \frac{\log(\Ncal/\delta)}{K}
\end{align}
\end{lemma}
\begin{proof}
    For any fixed $|f| \leq 1$, note that 
    \begin{align}
        &\frac{1}{K}\sum_{h=0}^{H-1}\sum_{k=1}^K \EE_{s\sim P^*(s_{h-1}^k, a_{h-1}^k), a \sim \pi^b(s)}f(s,a) - \sum_{h=0}^{H-1}\EE_{s,a\sim d^{\pi^b}_h} f(s,a)\notag \\
        & \leq \sum_{h=0}^{H-1} \frac{\text{vsr}_{s,a\sim d^{\pi^b}_h} f(s,a)}{\sqrt{K}}\log(1/\delta) + \frac{\log(1/\delta)}{K}
    \end{align}
    Taking union bound having our result. 
\end{proof}


% \wen{can we abstract the below long derivation into a lemma? so that later when bounding $C$ we can just call the lemma?}



% \wen{can we abstract the derivation for upper bounding $A$ below into a lemma as well? want to call this in the proof sketch in the main body.}

\section{New idea}
\begin{align}
    \pi^* =  \argmax_{\pi} \EE_{\rho^\pi}[\sum_{h=1}^H r_h]
\end{align}

have $\hat\rho$, 

\begin{align}
    \hat \pi = \argmax_{\pi} \EE_{\hat\rho}\prod_{h=1}^H\frac{\pi}{\pi^b} \sum_{h=1}^H r_h
\end{align}

\newpage
\section{Some questions about the online setting}
We can bound $V^{\pi^k}_{0;\widehat P^k}-V^{\pi^k}_{0;P^\star}$ using the simulation lemma (\pref{lem:simulation}):
\begin{align}
    V^{\pi^k}_{0;\widehat P^k}-V^{\pi^k}_{0;P^\star}&\leq \sum_{h=0}^{H-1} \EE_{s,a\sim d^{\pi^k}_h} \left[ \left|\EE_{s'\sim P^\star(s,a)} V^{\pi^k}_{h+1;\widehat P^k}(s') -\EE_{s'\sim \widehat P^k(s,a)} V^{\pi^k}_{h+1;\widehat P^k}(s')    \right|\right]. 
\end{align}
If we change the regret definition, we should be able to get the following:
\begin{equation}
    V^{\pi^k}_{0;\widehat P^k}-\sum_{s_h,a_h\in\tau_k}r_h(s_h,a_h)\leq \sum_{s_h,a_h\in\tau_k}  \left[ \left|\EE_{s'\sim P^\star(s_h,a_h)} V^{\pi^k}_{h+1;\widehat P^k}(s') -\EE_{s'\sim \widehat P^k(s_h,a_h)} V^{\pi^k}_{h+1;\widehat P^k}(s')    \right|\right]\label{1}\,,
\end{equation}
where $\tau_k$ is the executed trajectory using $\pi^k$ under $P^*$.

\textbf{Definitions:}
\begin{itemize}
    \item Let $\tau_k = (s_0, a_0, s_1, a_1, \dots, s_H)$ be the trajectory executed by policy $\pi^k$ under the true transition probabilities $P^*$.
    \item Let $V_{h; \hat{P}^k}^{\pi^k}(s)$ denote the value function at time step $h$ under policy $\pi^k$ and estimated transition probabilities $\hat{P}^k$.
\end{itemize}

\begin{equation} \begin{aligned} V^{\pi^k}_{0; \widehat{P}^k}(s_0) - \sum_{h=0}^{H-1} r_h(s_h, a_h) \leq \sum_{h=0}^{H-1} \left| \mathbb{E}_{s' \sim P^*(\cdot \mid s_h, a_h)} \left[ V^{\pi^k}_{h+1; \widehat{P}^k}(s') \right] - \mathbb{E}_{s' \sim \widehat{P}^k(\cdot \mid s_h, a_h)} \left[ V^{\pi^k}_{h+1; \widehat{P}^k}(s') \right] \right| \end{aligned} \label{eq
} \end{equation}
% Then what should the LHS be... And it has to be related to $V^{\pi^k}_{0;\widehat P^k}-V^{\pi^k}_{0;P^\star}$, otherwise how can we use the optimism? If there needs some concentration to make the connection, it may cause some poly dependence on H...

Then do we need the following MLE generalization bound (it is true by simply treating $D_i$ as a deterministic delta distribution)
\begin{equation}
    \sum_{i=0}^{k-1} \sum_{s,a\in\tau_i}   H^2(P^k(s ,a )||P^*(s ,a ))\leq \log(K|P|/\delta)
\end{equation}
% We have the following expected version
% \begin{equation}
%     \sum_{i=0}^{k-1} \sum_{h=1}^H E_{s_h\sim P^*(s_{h-1}^i,a_{h-1}^i),a_h\sim\pi^i} H^2(P^k(s_h,a_h)||P^*(s_h,a_h))\leq \log(K|P|/\delta)
% \end{equation}

% The previous one should be a weaker version.

Because to bound Eq.(\ref{1}), subsequently we need to further bound the following using eluder
\begin{align}
   \sum_{k=0}^{K-1}\sum_{s,a\in\tau^k}  \left[\big(\VV_{P^\star} V_{h+1; \widehat P^k}^{\pi^k}\big)(s,a)\right]\cdot\sum_{k=0}^{K-1}\sum_{s,a\in\tau^k}\left[\mathbb H^2\Big(P^\star(s,a)\Mid \widehat P^k\big(s,a)\Big)\right]
\end{align}

% But by MLE we have the following expectation version?
% \begin{equation}
%     \sum_{i=0}^{k-1} \sum_{h=1}^H E_{s_h\sim P^*(s_{h-1}^i,a_{h-1}^i),a_h\sim\pi^i} H^2(P^k(s_h,a_h)||P^*(s_h,a_h))\leq \log(K|P|/\delta)
% \end{equation}

One issue is applying the eluder in $N=HK$ steps to bound the term
\begin{align}
   \sum_{k=0}^{K-1}\sum_{s,a\in\tau^k}\left[\mathbb H^2\Big(P^\star(s,a)\Mid \widehat P^k\big(s,a)\Big)\right]
\end{align}

\begin{lemma}[modified Eluder Pigeonhole Lemma for N=HK]\label{lem:eluder-pigeonhole1}
Let $C := \sup_{(s,a)\in\Scal\times\Acal,f\in\Psi}\abs{ f((s,a))}$ be the envelope.
Fix any $K\in\NN$ and sequences $f^{(1)},\dots,f^{(N)}\subseteq \Psi$, $(s,a)^{(1)},\dots,(s,a)^{(N)}\subseteq\Scal\times\Acal$.
Let $\beta$ be a constant such that for all $n\in[N]$ we have,
$
    \sum_{i=0}^{\lfloor \frac{n-1}{H}\rfloor\cdot H}\abs{f^{(n)}((s,a)^i)} \leq \beta.
$
Then, for all $n\in[N]$ and n mod H=0, , we have
\begin{equation*}
    \sum_{t=1}^n\abs{f^{(t)}((s,a)^t)}\leq \inf_{0<\epsilon\leq 1}\braces{ \text{DE}_1(\Psi,\Dcal,\epsilon)(2C + \beta\log(C/\epsilon)) + n\epsilon }.
\end{equation*}
\end{lemma}

Is the above true?

If yes, then the remaining issue is the variance term 
\begin{align}
   \sum_{k=0}^{K-1}\sum_{s,a\in\tau^k}  \left[\big(\VV_{P^\star} V_{h+1; \widehat P^k}^{\pi^k}\big)(s,a)\right] 
\end{align}





\section{Proof to the modified E dimension}
For implicity, I use $x = (s,a)$. First, we need a new Eluder dimension definition. 
    \begin{definition}
        $DE_1(\Psi, \Scal \times \Acal, \epsilon)$ is the eluder dimension for $\Scal \times \Acal$ with function class $\Psi$, when the longest $\epsilon$-independent sequence $x^1,\dots, x^L$ enjoys the length less than $D(\epsilon)$, i.e.,  there exists $g \in \Psi$ such that $\sum_{l=1}^{L-1} |g(x^l)| \leq \epsilon$ and $|g(x^L)|>\epsilon$. 
    \end{definition}
    
Here we propose a new lemma. 
\begin{lemma}[Generalized Eluder Pigeonhole Lemma]\label{lem: generalized pigeonhole}
Let the event $\Ecal$ be 
\begin{align}
    \Ecal: \forall k \in [K],\ \sum_{i=1}^{k-1} \sum_{h=1}^H   H^2(P^k(s_h^i ,a_h^i )||P^*(s_h^i ,a_h^i ))\leq \log(K|P|/\delta)
\end{align}
Then under event $\Ecal$, there exists a set $\Kcal \in [K]$ such that
\begin{itemize}[leftmargin = *]
    \item We have $|\Kcal| \leq DE_1(\Psi, \Scal \times \Acal, \log(K|P|/\delta)/(KH))$
    \item We have
    \begin{align}
        &\sum_{k \in [K]\setminus \Kcal}\sum_{h=1}^H H^2\Big(P^\star(s_1^k,a_1^k)\Mid \widehat P^k\big(s_h^k,a_h^k)\Big)\notag \\
        &\leq \inf_{0<\epsilon\leq 1}\braces{ \text{DE}_1(\Psi,\Scal \times \Acal,\epsilon)(2 + 7\log(K|P|/\delta)\log(1/\epsilon)) + KH\epsilon }\notag \\
        & \leq 9\text{DE}_1(\Psi,\Scal \times \Acal,1/(KH))\cdot\log(K|P|/\delta)\log(KH)
    \end{align}
\end{itemize}
  
\end{lemma}

\subsection{Proof}




    
    We write $n = k\cdot H+h$, $k = 1,\dots, K$. Then we first prove the following claim:
    \begin{lemma}\label{lemma:zhou_1}
        Given $\lambda>0$. There exists at most $(D(\sqrt{\lambda/(KH)}) + 1)/2$ number of $k$ satisfying the following claim
        \begin{align}
        \sup_{g \in \Psi}\frac{\lambda + \sum_{k'=1}^{k}\sum_{h'=1}^H |g(x_{h'}^{k'})|}{\lambda + \sum_{k'=1}^{k-1}\sum_{h'=1}^H |g(x_{h'}^{k'})|} > 4.
\label{help:1}
        \end{align}
    \end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:zhou_1}]
    

Note that 
\begin{align}
   &\sum_{k=1}^K\min\bigg\{1, \log \sup_{g \in \Psi}\frac{\lambda + \sum_{k'=1}^{k}\sum_{h'=1}^H |g(x_{h'}^{k'})|}{\lambda + \sum_{k'=1}^{k-1}\sum_{h'=1}^H |g(x_{h'}^{k'})|} \bigg\}\notag \\
   &\leq \sum_{k=1}^K\min\bigg\{1,\log \prod_{h=1}^H \sup_{g \in \Psi}\frac{\lambda + \sum_{k'=1}^{k-1}\sum_{h'=1}^H |g(x_{h'}^{k'})| + \sum_{h'=1}^{h} |g(x_{h'}^{k})|}{\lambda + \sum_{k'=1}^{k-1}\sum_{h'=1}^H |g(x_{h'}^{k'})| + \sum_{h'=1}^{h-1} |g(x_{h'}^{k})|}\bigg\}\notag \\
   & = \sum_{k=1}^K\min\bigg\{1,\sum_{h=1}^H \log\bigg(1+ \sup_{g \in \Psi}\frac{|g(x_{h}^{k})|}{\lambda + \sum_{k'=1}^{k-1}\sum_{h'=1}^H |g(x_{h'}^{k'})| + \sum_{h'=1}^{h-1} |g(x_{h'}^{k})|}\bigg)\bigg\}\notag \\
   & \leq \sum_{k=1}^K\sum_{h=1}^H \min\bigg\{1,\sup_{g \in \Psi}\frac{|g(x_{h}^{k})|}{\sum_{k'=1}^{k-1}\sum_{h'=1}^H |g(x_{h'}^{k'})| + \sum_{h'=1}^{h-1} |g(x_{h'}^{k})| + \lambda}\bigg\}
\end{align}
where the first inequality holds since $\sup_x \prod_{i=1}^n f_i(x) \leq \prod_{i=1}^n \sup_x f_i(x)$ when $f_i\geq 1$, the second one holds since $\log(1+x) \leq x$ when $x>0$. To further bound it, we have the following lemma. 



\begin{lemma}
    We have
    \begin{align}
        \sum_{k=1}^K\sum_{h=1}^H \min\bigg\{1,\sup_{g \in \Psi}\frac{|g(x_{h}^{k})|}{\sum_{k'=1}^{k-1}\sum_{h'=1}^H |g(x_{h'}^{k'})| + \sum_{h'=1}^{h-1} |g(x_{h'}^{k})| + \lambda}\bigg\} \leq DE_1(\Psi, \Scal \times \Acal, \lambda/(KH)) + 1.\notag
    \end{align}
\end{lemma}
\begin{proof}
    Set $\epsilon$ to be some constant. Then by the definition of Eluder dimension, there are at most $DE_1(\Psi, \Scal \times \Acal, \epsilon)$ number of indices $k_i, h_i, i \in [DE_1(\Psi, \Scal \times \Acal, \epsilon)]$, satisfying
    \begin{align}
        \bigg(\exists g\in \Psi,\ \sum_{k=1}^{k_i-1}\sum_{h=1}^{H} |g(x_h^k)|  + \sum_{h=1}^{h_i - 1}|g(x_h^k)| \leq \epsilon,\ g(x_{h_i}^{k_i})>\epsilon\bigg)\Rightarrow \bigg(\sup_{g \in \Psi}\frac{|g(x_{h_i}^{k_i})|}{\sum_{k'=1}^{k_i-1}\sum_{h'=1}^H |g(x_{h'}^{k'})| + \sum_{h'=1}^{h_i-1} |g(x_{h'}^{k})| + \lambda} \geq \frac{\epsilon}{\epsilon+\lambda}\bigg).\notag
    \end{align}
    Therefore, let $\Hcal$ to be the collection of all above $k_i, h_i$, then we have
    \begin{align}
        &\sum_{k=1}^K\sum_{h=1}^H \min\bigg\{1,\sup_{g \in \Psi}\frac{|g(x_{h}^{k})|}{\sum_{k'=1}^{k-1}\sum_{h'=1}^H |g(x_{h'}^{k'})| + \sum_{h'=1}^{h-1} |g(x_{h'}^{k})| + \lambda}\bigg\}\notag \\
        & \leq \sum_{(k,h) \in \Hcal}1 + \sum_{(k,h) \notin \Hcal}\frac{\epsilon}{\epsilon+\lambda}\notag \\
        & \leq DE_1(\Psi, \Scal \times \Acal, \epsilon) + \frac{\epsilon\cdot KH}{\epsilon+\lambda}.
    \end{align}
    Then taking $\epsilon = \lambda/KH$ guarantees our statement. 
\end{proof}


Therefore, we have at most $(DE_1(\Psi, \Scal \times \Acal, \lambda/(KH)) + 1)/2$ number of $k$ satisfying
\begin{align}
    \min\bigg\{1, \log \sup_{g \in \Psi}\frac{\lambda + \sum_{k'=1}^{k}\sum_{h'=1}^H |g(x_{h'}^{k'})|}{\lambda + \sum_{k'=1}^{k-1}\sum_{h'=1}^H |g(x_{h'}^{k'})|} \bigg\} \geq 2,
\end{align}
which suggests the proposition. 

\end{proof}

Let all the $k$ not satisfying Lemma \ref{lemma:zhou_1} be the set $\Kcal$. Then for all $k \in \Kcal$, suppose $n = kH+h$, then we will have the following with $\lambda = \beta$: 
\begin{align}
    \sum_{i=0}^{n-1}\abs{f^{(n)}((s,a)^i)} \leq \sum_{i=0}^{kH+H}\abs{f^{(n)}((s,a)^i)} \leq 3\lambda + 4(\sum_{i=0}^{\lfloor \frac{n-1}{H}\rfloor\cdot H}\abs{f^{(n)}((s,a)^i)} ) = 7\beta
\end{align}
which satisfies the Lemma 12 reuiqrement. For all the $k \notin \Kcal$, you directly bound the regret at episode $k$ by 1. Since the $|[K]\setminus \Kcal| \leq (DE_1(\Psi, \Scal \times \Acal, \lambda/(KH)) + 1)/2 \leq DE_1(\Psi, \Scal \times \Acal, \beta/(KH))$, it only contributes additional $D$ to the total regret, which is fine. 




\section{Decomposition}
 
% \begin{align}
%     &V^{\pi^k}_{0;\widehat P^k}(s_1^k)-V^{\pi^k}_{0;P^\star} (s_1^k) \notag \\
%     &= Q^{\pi^k}_{0;\widehat P^k}(s_1^k, a_1^k)-Q^{\pi^k}_{0;P^\star} (s_1^k, a_1^k)\notag \\
%     & = \EE_{s'\sim \widehat P^k(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s') - \EE_{s'\sim P^*(s_1^k, a_1^k)}V^{\pi^k}_{1;P^*}(s')\notag \\
%     & = \EE_{s'\sim P^*(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s') - \EE_{s'\sim P^*(s_1^k, a_1^k)}V^{\pi^k}_{1;P^*}(s') + \EE_{s'\sim \widehat P^k(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s') - \EE_{s'\sim P^*(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s')\notag \\
%     & = V^{\pi^k}_{1;\widehat P^k}(s_2^k)-V^{\pi^k}_{1;P^\star} (s_2^k) + \underbrace{\EE_{s'\sim P^*(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s') - \EE_{s'\sim P^*(s_1^k, a_1^k)}V^{\pi^k}_{1;P^*}(s') - (V^{\pi^k}_{1;\widehat P^k}(s_2^k)-V^{\pi^k}_{1;P^\star} (s_2^k))}_{I_1^k}\notag \\
%     &\quad + \EE_{s'\sim \widehat P^k(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s') - \EE_{s'\sim P^*(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s')\notag \\
%     & \leq  V^{\pi^k}_{1;\widehat P^k}(s_2^k)-V^{\pi^k}_{1;P^\star} (s_2^k) + I_1^k + \sqrt{\big(\VV_{P^\star} V_{1; \widehat P^k}^{\pi^k}\big)(s_1^k,a_1^k)\mathbb H^2\Big(P^\star(s,a)\Mid \widehat P^k\big(s,a)\Big)}
% \end{align}

% Therefore we have
% \begin{align}
%     V^{\pi^k}_{0;\widehat P^k}(s_1^k)-V^{\pi^k}_{0;P^\star} (s_1^k) \leq \sum_{h=1}^H I_h^k + \sum_{h=1}^H\sqrt{\big(\VV_{P^\star} V_{h; \widehat P^k}^{\pi^k}\big)(s_h^k,a_h^k)\mathbb H^2\Big(P^\star(s,a)\Mid \widehat P^k\big(s,a)\Big)}
% \end{align}

% Next we bound $I_1^k$. 


Suppose we have a deterministic policy $\pi^k$.
\begin{align}
    &V^{\pi^k}_{0;\widehat P^k}(s_1^k)-\sum_{h=1}^H r(s_h^k, a_h^k) \notag \\
    &= Q^{\pi^k}_{0;\widehat P^k}(s_1^k, a_1^k)-\sum_{h=1}^H r(s_h^k, a_h^k)\notag \\
    & = \EE_{s'\sim \widehat P^k(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s') - \sum_{h=2}^H r(s_h^k, a_h^k)\notag \\
    & = \EE_{s'\sim P^*(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s') - \sum_{h=2}^H r(s_h^k, a_h^k) + \EE_{s'\sim \widehat P^k(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s') - \EE_{s'\sim P^*(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s')\notag \\
    & = V^{\pi^k}_{1;\widehat P^k}(s_2^k)-\sum_{h=2}^H r(s_h^k, a_h^k) + \underbrace{\EE_{s'\sim P^*(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s')  - V^{\pi^k}_{1;\widehat P^k}(s_2^k)}_{I_1^k}\notag \\
    &\quad + \EE_{s'\sim \widehat P^k(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s') - \EE_{s'\sim P^*(s_1^k, a_1^k)}V^{\pi^k}_{1;\widehat P^k}(s')\notag \\
    & \leq  V^{\pi^k}_{1;\widehat P^k}(s_2^k)-\sum_{h=2}^H r(s_h^k, a_h^k) + I_1^k + \sqrt{\big(\VV_{P^\star} V_{1; \widehat P^k}^{\pi^k}\big)(s_1^k,a_1^k)\mathbb H^2\Big(P^\star(s_1^k,a_1^k)\Mid \widehat P^k\big(s_h^k,a_h^k)\Big)}\notag\\
    &+H^2\Big(P^\star(s_1^k,a_1^k)\Mid \widehat P^k\big(s_h^k,a_h^k)\Big)
\end{align}

Therefore we have
\begin{align}
    \sum_{k=1}^K(V^{\pi^k}_{0;\widehat P^k}(s_1^k)-\sum_{h=1}^H r(s_h^k, a_h^k)) &\leq \sum_{k=1}^K\sum_{h=1}^H I_h^k + \sum_{k=1}^K\sum_{h=1}^H\sqrt{\big(\VV_{P^\star} V_{h; \widehat P^k}^{\pi^k}\big)(s_h^k,a_h^k)\mathbb H^2\Big(P^\star(s_h^k,a_h^k)\Mid \widehat P^k\big(s_h^k,a_h^k)\Big)}\notag\\
    &+\sum_{k=1}^K\sum_{h=1}^HH^2\Big(P^\star(s_1^k,a_1^k)\Mid \widehat P^k\big(s_h^k,a_h^k)\Big)
\end{align}

Next we bound $I_h^k$. Note that by Bernstein, 
\begin{align}
    \sum_{k=1}^K \sum_{h=1}^H I_h^k\leq \sqrt{\sum_{k=1}^K \sum_{h=1}^H \big(\VV_{P^\star} V_{h; \widehat P^k}^{\pi^k}\big)(s_h^k,a_h^k)} + O(1)\log(1/\delta)
\end{align}

Then we should be able to follow the original steps. 

\begin{align}
&\sum_{k=1}^K\sum_{h=1}^H\sqrt{\big(\VV_{P^\star} V_{h; \widehat P^k}^{\pi^k}\big)(s_h^k,a_h^k)\mathbb H^2\Big(P^\star(s_h^k,a_h^k)\Mid \widehat P^k\big(s_h^k,a_h^k)\Big)}\notag\\
&\leq\sqrt{\sum_{k=1}^K\sum_{h=1}^H\big(\VV_{P^\star} V_{h; \widehat P^k}^{\pi^k}\big)(s_h^k,a_h^k)\sum_{k=1}^K\sum_{h=1}^HH^2\Big(P^\star(s_1^k,a_1^k)\Mid \widehat P^k\big(s_h^k,a_h^k)\Big)}
\end{align}
By the MLE generalization bound, we have
\begin{equation}
    \sum_{i=0}^{k-1} \sum_{h=1}^H   H^2(P^k(s_h^i ,a_h^i )||P^*(s_h^i ,a_h^i ))\leq \log(K|P|/\delta)
\end{equation}
By Lemma\ref{lem:eluder-pigeonhole1}, we have
\begin{equation}
\sum_{k=1}^K\sum_{h=1}^HH^2\Big(P^\star(s_1^k,a_1^k)\Mid \widehat P^k\big(s_h^k,a_h^k)\Big)\lesssim \dimRL\log(K|P|/\delta)
\end{equation}

Then what remains is to bound $\sum_{k=1}^K\sum_{h=1}^H\big(\VV_{P^\star} V_{h+1; \widehat P^k}^{\pi^k}\big)(s_h^k,a_h^k)$ with $\sum_{k=1}^K\sum_{h=1}^H\big(\VV_{P^\star} V_{h+1}^{\pi^k}\big)(s_h^k,a_h^k)$

For notational simplicity, we denote 
\begin{align}
    &A:=\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\big(\VV_{P^\star} V_{h+1; \widehat P^k}^{\pi^k}\big)(s_h^k,a_h^k)\right]\notag\\
    &B:=\sum_{k=0}^{K-1}\sum_{h=0}^{H-1}\left[\big(\VV_{P^\star} V_{h+1}^{\pi^k}\big)(s_h^k,a_h^k)\right],\notag\\
    &C:=\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\big(\VV_{P^\star}( V_{h+1; \widehat P^k}^{\pi^k}-V_{h+1}^{\pi^k})\big)(s_h^k,a_h^k)\right],\notag
\end{align}
then we have $A\leq 2B+2C$ since $\VV_{P^\star}(a+b)\leq 2\VV_{P^\star}(a)+2\VV_{P^\star}(b)$.
% $A_1:=\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \EE_{s,a \sim d^{\pi^k}_h}\left[\big(\VV_{P^\star} V_{h+1; \widehat P^k}^{\pi^k}\big)(s,a)\right]$, and we denote
% $B_1:=\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \EE_{s,a \sim d^{\pi^k}_h}\left[\big(\VV_{P^\star} V_{h+1}^{\pi^k}\big)(s,a)\right]$, $C_1:=\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \EE_{s,a \sim d^{\pi^k}_h}\left[\big(\VV_{P^\star}( V_{h+1; \widehat P^k}^{\pi^k}-V_{h+1}^{\pi^k})\big)(s,a)\right]$, 


Let $\Delta_{h+1}^{\pi^k}:=V_{h+1; \widehat P^k}^{\pi^k}-V_{h+1}^{\pi^k}$. Then, we have
\begin{align}
    C&=\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\big(P^\star(\Delta_{h+1}^{\pi^k})^2\big)(s_h^k,a_h^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big)^2(s_h^k,a_h^k)\right]\notag\\
    &=\sum_{k=0}^{K-1}\sum_{h=0}^{H-1}\left[(\Delta_{h+1}^{\pi^k})^2(s_{h+1}^k)\right]-\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\big(P^\star\Delta_{h+1}^{\pi^k}\big)^2(s_h^k,a_h^k)\right]+\sum_k\sum_h \left(\EE_{s\sim P^*(s_h^k,a_h^k)}\left[(\Delta_{h+1}^{\pi^k})^2(s)\right]-(\Delta_{h+1}^{\pi^k})^2(s_{h+1}^k)\right)\notag\\
    &\leq \sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[(\Delta_{h}^{\pi^k})^2(s_{h+1}^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big)^2(s_h^k,a_h^k)\right]+\sum_k\sum_h \Gamma_{h,k}\notag\\
    &\leq \sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[(\Delta_{h}^{\pi^k})^2(s_{h+1}^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big)^2(s_h^k,a_h^k)\right]+\sqrt{\sum_k\sum_h \VV_{P^*}\left((V_{h+1; \widehat P^k}^{\pi^k}-V_{h+1}^{\pi^k})^2\right)(s_h^k,a_h^k)}+O(1)\log(1/\delta)\notag\\
    &=\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\Big((\Delta_{h}^{\pi^k})(s_{h+1}^k)+\big(P^\star\Delta_{h+1}^{\pi^k}\big)(s_h^k,a_h^k)\Big)\cdot\Big((\Delta_{h}^{\pi^k})(s_{h+1}^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big)(s_h^k,a_h^k)\Big)\right]\notag\\
    &+\sqrt{\sum_k\sum_h \VV_{P^*}\left((V_{h+1; \widehat P^k}^{\pi^k}-V_{h+1}^{\pi^k})^2\right)(s_h^k,a_h^k)}+\log(1/\delta)\notag\\
    &\leq 2 \sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\left|(\Delta_{h}^{\pi^k})(s_{h+1}^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big)(s_h^k,a_h^k)\right|\right]+\sqrt{\sum_k\sum_h \VV_{P^*}\left((V_{h+1; \widehat P^k}^{\pi^k}-V_{h+1}^{\pi^k})^2\right)(s_h^k,a_h^k)}+\log(1/\delta)\label{eqn: help 10}
\end{align}We have
\begin{align}
&2 \sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\left|(\Delta_{h}^{\pi^k})(s_{h+1}^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big)(s_h^k,a_h^k)\right|\right] \\
    &=2 \sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\left|({V}_{h;\widehat P^k}^{\pi^k})(s_{h+1}^k)-\big(P^\star{V}_{h+1;\widehat P^k}^{\pi^k}\big)(s_h^k,a_h^k)-\Big(({V}_{h}^{\pi^k})(s_{h+1}^k)-\big(P^\star{V}_{h+1}^{\pi^k}\big)(s_h^k,a_h^k)\Big)\right|\right]\notag\\
    &=2 \sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\left|r(s_h^k,a_h^k)+\big(\widehat P^k{V}_{h+1;\widehat P^k}^{\pi^k}\big)(s_h^k,a_h^k)-\big(P^\star{V}_{h+1;\widehat P^k}^{\pi^k}\big)(s_h^k,a_h^k)-r(s_h^k,a_h^k)\right|\right]\notag\\
        &=2 \sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\left|\big(\widehat P^k{V}_{h+1;\widehat P^k}^{\pi^k}\big)(s_h^k,a_h^k)-\big(P^\star{V}_{h+1;\widehat P^k}^{\pi^k}\big)(s_h^k,a_h^k)\right|\right]\notag\\
        &= 2 \sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\left|\EE_{s'\sim P^\star(s_h^k,a_h^k)}\left[V^{\pi^k}_{h+1;\widehat P^k}(s')\right]-\EE_{s'\sim\widehat P^k(s_h^k,a_h^k)}\left[V^{\pi^k}_{h+1;\widehat P^k}(s')\right]\right|\right]\notag\\
        &\leq 16 \sqrt{ \sum_{k=1}^K\sum_{h=1}^H\big(\VV_{P^\star} V_{h; \widehat P^k}^{\pi^k}\big)(s_h^k,a_h^k)\cdot 88\dimRL\log(\left|\Pcal\right|/\delta)\log(K)}+3520\dimRL\log(K\left|\Pcal\right|/\delta)\log(K)\notag\\
        &=16 \sqrt{A\cdot 88\dimRL\log(\left|\Pcal\right|/\delta)\log(K)}+3520\dimRL\log(K\left|\Pcal\right|/\delta)\log(K)\label{eqn: help 11}
\end{align}
 where the first equality is by the definition of $\Delta_{h+1}^{\pi^k}$, the second equality is because $a$ is drawn from $\pi^k$, the inequality holds with probability at least $1-\delta$ by \pref{lem: online sum mean value difference}, and the last equality is by definition of $A_1$.

Then substituting \pref{eqn: help 11} into \pref{eqn: help 10}, we obtain an upper bound for $C_1$, which suggests
\begin{align}
    A&\leq 2B+2C\notag\\
    &\leq 2B+7040\dimRL\log(K\left|\Pcal\right|/\delta)\log(K)+\sqrt{\sum_k\sum_h \VV_{P^*}\left((V_{h+1; \widehat P^k}^{\pi^k}-V_{h+1}^{\pi^k})^2\right)(s_h^k,a_h^k)}\notag\\
    &+\quad32\sqrt{88\dimRL\log(K\left|\Pcal\right|/\delta)\log(K)}\cdot\sqrt{A}.\notag
\end{align}
Then, with the fact that $x\leq 2a+b^2$ if $x\leq a+b\sqrt{x}$, we have
\begin{align}
    A&\leq 4B+14080\dimRL\log(K\left|\Pcal\right|/\delta)\log(K)+\sqrt{\sum_k\sum_h \VV_{P^*}\left((V_{h+1; \widehat P^k}^{\pi^k}-V_{h+1}^{\pi^k})^2\right)(s_h^k,a_h^k)}+90112\dimRL\log(K\left|\Pcal\right|/\delta)\log(K)\notag \\
    &\leq  O(B+\dimRL \log(K\left|\Pcal\right|/\delta)\log(K))+\sqrt{\sum_k\sum_h \VV_{P^*}\left((V_{h+1; \widehat P^k}^{\pi^k}-V_{h+1}^{\pi^k})^2\right)(s_h^k,a_h^k)}.\notag
\end{align}

When what remains is to bound $\sqrt{\sum_k\sum_h \VV_{P^*}\left((V_{h+1; \widehat P^k}^{\pi^k}-V_{h+1}^{\pi^k})^2\right)(s_h^k,a_h^k)}$.


For notational simplicity, let us denote
\begin{align}
   C_m&:=\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\big(\VV_{P^\star}( V_{h+1; \widehat P^k}^{\pi^k}-V_{h+1}^{\pi^k})^{2^m}\big)(s_h^k,a_h^k)\right]\notag\\
    G&:=\sqrt{A\cdot\dimRL\log(K|\Pcal|/\delta)}+\dimRL\log(K|\Pcal|/\delta)
\end{align}
We have $\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\left|(\Delta_{h}^{\pi^k})(s_{h+1}^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big)(s_h^k,a_h^k)\right|\right]\leq G$, and $C_0\lesssim 2G+\sqrt{C_1}$. Now we want to bound $C_0$. We have the following 
\begin{align}
    C_m&=\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\big(P^\star(\Delta_{h+1}^{\pi^k})^{2^{m+1}}\big)(s_h^k,a_h^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big)^{2^{m+1}}(s_h^k,a_h^k)\right]\notag\\
    &=\sum_{k=0}^{K-1}\sum_{h=0}^{H-1}\left[(\Delta_{h+1}^{\pi^k})^{2^{m+1}}(s_{h+1}^k)\right]-\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\big(P^\star\Delta_{h+1}^{\pi^k}\big)^{2^{m+1}}(s_h^k,a_h^k)\right]\notag\\
    &\quad+\sum_k\sum_h \left(\EE_{s\sim P^*(s_h^k,a_h^k)}\left[(\Delta_{h+1}^{\pi^k})^{2^{m+1}}(s)\right]-(\Delta_{h+1}^{\pi^k})^{2^{m+1}}(s_{h+1}^k)\right)\notag\\
    &\leq \sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[(\Delta_{h}^{\pi^k})^{2^{m+1}}(s_{h+1}^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big)^{2^{m+1}}(s_h^k,a_h^k)\right]+\sum_k\sum_h \Gamma_{h,k}\notag\\
    &\leq \sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[(\Delta_{h}^{\pi^k})^{2^{m+1}}(s_{h+1}^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big)^{2^{m+1}}(s_h^k,a_h^k)\right]+\sqrt{\sum_k\sum_h \VV_{P^*}\left((V_{h+1; \widehat P^k}^{\pi^k}-V_{h+1}^{\pi^k})^{2^{m+1}}\right)(s_h^k,a_h^k)}+\log(1/\delta)\notag\\
    &=\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\Big((\Delta_{h}^{\pi^k})^{2^m}(s_{h+1}^k)+\big(P^\star\Delta_{h+1}^{\pi^k}\big)^{2^m}(s_h^k,a_h^k)\Big)\cdot\Big((\Delta_{h}^{\pi^k})^{2^m}(s_{h+1}^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big)^{2^m}(s_h^k,a_h^k)\Big)\right] 
    +\sqrt{C_{m+1}}+\log(1/\delta)\notag\\
    &\leq 2 \sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\left|(\Delta_{h}^{\pi^k})^{2^{m-1}}(s_{h+1}^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big){2^{m-1}}(s_h^k,a_h^k)\right|\right]+\sqrt{C_{m+1}}\notag\\
    &=2 \left[\Big((\Delta_{h}^{\pi^k})^{2^{m-2}}(s_{h+1}^k)+\big(P^\star\Delta_{h+1}^{\pi^k}\big)^{2^{m-2}}(s_h^k,a_h^k)\Big)\cdot\Big((\Delta_{h}^{\pi^k})^{2^{m-2}}(s_{h+1}^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big)^{2^{m-2}}(s_h^k,a_h^k)\Big)\right] +\sqrt{C_{m+1}}+\log(1/\delta)\notag\\
    &\leq 2^2\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\left|(\Delta_{h}^{\pi^k})^{2^{m-2}}(s_{h+1}^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big)^{2^{m-2}}(s_h^k,a_h^k)\right|\right]+\sqrt{C_{m+1}}\notag\\
    &\leq 2^{m+1}\sum_{k=0}^{K-1}\sum_{h=0}^{H-1} \left[\left|(\Delta_{h}^{\pi^k}) (s_{h+1}^k)-\big(P^\star\Delta_{h+1}^{\pi^k}\big) (s_h^k,a_h^k)\right|\right]+\sqrt{C_{m+1}}+\log(1/\delta)\notag\\
    &\lesssim 2^{m+1}G+\sqrt{C_{m+1}}
    \label{eqn: help 10}
\end{align}
Therefore, assume that $G\geq 2$, we have
\begin{align}
    C_0\leq 4G.
\end{align}
 We have the following lemma to prove the above result

